Whispers of Many Shores: Cultural Alignment through Collaborative Cultural Expertise

The integration of large language models (LLMs) into global applications necessitates effective cultural alignment for meaningful and culturally-sensitive interactions. Current LLMs often lack the nuanced understanding required for diverse cultural contexts, and adapting them typically involves costly full fine-tuning. To address this, we introduce a novel soft prompt fine-tuning framework that enables efficient and modular cultural alignment. Our method utilizes vectorized prompt tuning to dynamically route queries to a committee of culturally specialized 'expert' LLM configurations, created by optimizing soft prompt embeddings without altering the base model's parameters. Extensive experiments demonstrate that our framework significantly enhances cultural sensitivity and adaptability, improving alignment scores from 0.208 to 0.820, offering a robust solution for culturally-aware LLM deployment. This research paves the way for subsequent investigations into enhanced cultural coverage and dynamic expert adaptation, crucial for realizing autonomous AI with deeply nuanced understanding in a globally interconnected world.

==> SeparateSection/Abstruct.tex <==
\begin{abstract}
% The integration of large language models (LLMs) into global applications necessitates effective cultural alignment to ensure meaningful and culturally-sensitive interactions. Languages such as Chinese introduce unique challenges due to the frequent occurrence of adjectives with multiple context-dependent meanings, leading to diverse and nuanced interpretations. Additionally, Chinese linguistic humor heavily relies on rhyming and wordplay, which significantly differs from English humor, often characterized by puns, homophones, or deliberate silence for comedic effect. In this study, we introduce a novel soft prompt fine-tuning framework specifically designed for cultural alignment. By dynamically selecting and routing queries through culturally specialized experts using vectorized prompt tuning, our method efficiently optimizes prompt embeddings without altering the model's underlying parameters. Extensive experiments demonstrate that our approach significantly enhances cultural sensitivity and adaptability, providing an efficient and robust solution for culturally-aware language model deployment.

The integration of large language models (LLMs) into global applications necessitates effective cultural alignment for meaningful and culturally-sensitive interactions.  Current LLMs often lack the nuanced understanding required for diverse cultural contexts, and adapting them typically involves costly full fine-tuning. To address this, we introduce a novel soft prompt fine-tuning framework that enables efficient and modular cultural alignment. Our method utilizes vectorized prompt tuning to dynamically route queries to a committee of culturally specialized 'expert' LLM configurations, created by optimizing soft prompt embeddings without altering the base model's parameters. Extensive experiments demonstrate that our framework significantly enhances cultural sensitivity and adaptability, improving alignment scores from 0.208 to 0.820 (cf.Table~\ref{tab:model_comparison}), offering a robust solution for culturally-aware LLM deployment. This research paves the way for subsequent investigations into enhanced cultural coverage and dynamic expert adaptation, crucial for realizing autonomous AI with deeply nuanced understanding in a globally interconnected world.
% \textbf{[update evaluation metrics and results here,future outlook here]}
\end{abstract}
